Weakly Supervised Few-Shot Segmentation Via Meta-Learning

Semantic segmentation is a classic computer vision task with multiple applications, which includes medical and remote sensing image analysis. Despite recent advances with deep-based approaches, labeling samples (pixels) for training models is laborious and, in some cases, unfeasible. In this paper, we present two novel meta learning methods, named WeaSeL and ProtoSeg, for the few-shot semantic segmentation task with sparse annotations. We conducted extensive evaluation of the proposed methods in different applications (12 datasets) in medical imaging and agricultural remote sensing, which are very distinct fields of knowledge and usually subject to data scarcity. The results demonstrated the potential of our method, achieving suitable results for segmenting both coffee/orange crops and anatomical parts of the human body in comparison with full dense annotation.

==> results/results_old.tex <==
\section{Results and Discussion}\label{chap:results}

In this chapter we present the results of our experiments and a brief discussion about it. We grouped the experiments by research questions that motivate it. First, in Section~\ref{sec:sparse_v_dense}, we compare the results of the methods and baselines using multiple sparse annotations and their versions using dense labels. In Section~\ref{sec:sparse_comparison} we compare different sparse annotations in relation to the number of inputs that an user gives and the score obtained. %Finally, in Section~\ref{sec:adapt_time} we compare the number of epochs of fine tuning the few-shot task and the score of our methods. 

\subsection{Few-shot Semantic Segmentation: Sparse vs Dense labels}\label{sec:sparse_v_dense}
In this section we present the results of our methods in multiple few-shot tasks in the Medical and Remote Sensing scenarios. We vary the number of shots, and for each type of sparse annotation we vary their parameters as well.

With these experiments we answer our first research question about the impact of using sparse annotations in scenarios few-shot. Also, since we use multiple types of sparse annotations in the experiments, we can visualize how the different styles perform with the evaluated methods.

We will only present some of the results in this section. As a rule for \textit{this section}, we present the results grouped in graphs by sparse annotation type and number of shots. Dashed lines in the graphs are the scores of the methods trained with dense annotations. %Additional results can be seen in the Appendix~\ref{appendix:ex_results}.

\subsubsection{Medical Tasks}\label{sec:med_results}

We divided the medical results by the type of images of the tasks.

\textbf{1.A Chest X-Ray Datasets: }
For the evaluated CRX Datasets Tasks (\ref{sec:med_datasets} [1.A - 1.E]) we observed a tendency in the results. First, the obvious one that holds for, practically, all methods and scenarios, is that with more data better scores are obtained. That is, with large support sets (higher $k$-shots) and more sparse labeled pixels the models predicted more precise segmentations. 

A second observed result is that the \mamlmethod method appears to be the best approach to tasks with a significant discrepancy to other tasks in their category. We observed this in the \textit{JSRT Lungs} (Figure~\ref{fig:jsrt_lungs_results}) and the \textit{JSRT Heart} (Figure~\ref{fig:jsrt_heart_results}). The JSRT dataset is visually the most different of the CRX datasets. Moreover, the \textit{Heart} class is only present in this dataset, so this task does not have a direct parallel in other datasets.

\newcommand{\currprop}{0.85\textwidth}

% \subsubsection{JSRT: Lungs}
% \def\svgwidth{\currprop}
% \input{results/figs/jsrt_lungs_results_v2.pdf_tex}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/jsrt_lungs_results_v2.pdf}
    \caption{Jaccard Score of experiments with JSRT Lungs Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:jsrt_lungs_results}
\end{figure*}
% Results JSRT lungs.

% \subsubsection{JSRT: Hearts}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/jsrt_heart_results_v2.pdf}
    \caption{Jaccard Score of experiments with JSRT Heart Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:jsrt_heart_results}
\end{figure*}
% Results JSRT Hearts.

For the remainder tasks, we observe that either the \protomethod method or some Fine-tuning baseline is the best performer. Since some datasets are similar visually, fine-tuning for a task from a model trained in a similar dataset is a known viable solution that works well in these cases. These results are visible for the \textit{OpenIST, Montgomery}, and \textit{NIH-Labeled Lungs} tasks (Figures~\ref{fig:openist_lungs_results}, \ref{fig:montgomery_lungs_results}, and~\ref{fig:nih_labeled_lungs_results}, respectively). Fine-tuning from similar tasks (OpenIST, Shenzhen, or Montgomery) yields the best jaccard scores in most cases. Also, we observe that the \protomethod is consistently comparable to these fine-tuned baselines.  

% \subsubsection{OpenIST: Lungs}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/openist_lungs_results_v2.pdf}
    \caption{Jaccard Score of experiments with OpenIST Lungs Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:openist_lungs_results}
\end{figure*}
% Results OpenIST lungs.

% \subsubsection{Montgomery: Lungs}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/montgomery_lungs_results_v2.pdf}
    \caption{Jaccard Score of experiments with Montgomery Lungs Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:montgomery_lungs_results}
\end{figure*}
% Results Montgomery lungs.

% \subsubsection{NIH-Labeled: Lungs}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/nih_labeled_lungs_results_v2.pdf}
    \caption{Jaccard Score of experiments with NIH-Labeled Lungs Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:nih_labeled_lungs_results}
\end{figure*}
% Results NIH-Labeled lungs.

We observe that the methods, as expected, tend to approach their score obtained when trained with dense labels as the sparsity of the annotation decrease. But, even in yet extremely sparse scenarios, such as $20$-points annotation that represent less then $1\%$ of the total pixels in the image, the gap between the methods trained on sparse annotations and their dense label versions is small, as can be seen in most of the experiments. The \mamlmethod method often achieve the same results with dense annotations when using sparse annotations for tuning. However, the only method that practically is indifferent to the type or sparsity of the annotations is the \protomethod method. Since the method takes the average of the features of labeled pixels to produce the class prototypes, if the embedding function is learned properly, the increase or decrease of labeled pixels will have little effect in the average vector. Increasing this number will only make the mean tend to the average vector of the dense case. Thus, as will be seen in the other experiments, the \protomethod method will mostly have a constant score across different tasks settings. 

These results seems to show that, given proper training time, the \mamlmethod can exploit the information of different tasks and provide a good starting point for fine-tuning. Additionally, the \protomethod method, albeit being designed to learn an unbiased ensemble function, benefit from similar tasks in the training distribution and seem to assimilate information of these tasks, thus performing better in similar cases. We have this assumption for the \protomethod method, because, excluding the JSRT Lungs class, 5 out 12 training tasks are a similar CRX Lung task. If uniformly distributed, approximately 40\% of the time one of these tasks will be selected for a meta-training epoch.


\textbf{1.B Mammography X-Ray Datasets: }
In the MRX Datasets Tasks (\ref{sec:med_datasets} [1.G - 1.H]), we see similar tendencies as in the CRX Datasets. Again, fine-tuning from similar tasks appears as a solid solution, with \mamlmethod method, in most cases, obtaining comparable results.

In the \textit{MIAS Breast} task (Figure~\ref{fig:mias_breast_results}), fine-tuning from the \textit{INbreast Breast} task is the best approach. In the more challenging \textit{INbreast Pectoral Muscle} task (Figure~\ref{fig:inbreast_pectoral_results}), the pre-training using the INbreast Dataset, provided the best starting weights for fine tuning. Since the objects (Pectoral Muscle) in this target class are small (relative to breast, or lungs, for example), being used to the visual of the data seems to be more relevant to the model than the knowledge of the object in other dataset. 

The \protomethod method seems consistent in the \textit{MIAS Breast} task (Figure~\ref{fig:mias_breast_results}), with few variances across different task settings. In the \textit{INbreast Pectoral Muscle} task (Figure~\ref{fig:inbreast_pectoral_results}), given the difference of most methods to their dense labeled trained versions, we assume that the combination of the few-shot samples and, subsequently, generated sparse annotations were not informative enough, specially in the Contour Type annotation scenario.

% \subsubsection{MIAS: Breasts}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/mias_breast_results_v2.pdf}
    \caption{Jaccard Score of experiments with MIAS Breast Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:mias_breast_results}
\end{figure*}
% Results MIAS Breasts.

% \subsubsection{INbreast: Pectoral Muscle}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/inbreast_pectoral_results_v2.pdf}
    \caption{Jaccard Score of experiments with INbreast Pectoral Muscle Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:inbreast_pectoral_results}
\end{figure*}
% Results INbreast Pectoral Muscle.

\textbf{1.C Dental X-Ray Datasets: }
Once more, for the DRX Datasets Tasks (\ref{sec:med_datasets} [1.I - 1.J]), we observed the same trend for the evaluated approaches.

This time, without a similar task to fine-tune from, the \mamlmethod show to be the best performer, achieving the highest scores in most of the cases, with both dense and sparse annotations. This is observed in the \textit{Panoramic Mandible} task (Figure~\ref{fig:panoramic_mandible_results}) and the \textit{UFBA-UESC Teeth} task (Figure~\ref{fig:ufba_teeth_results}). Being the most distinct tasks, even the From Scratch baseline, provides satisfying results, and in some cases is the best model. 

% \subsubsection{Panoramic: Mandible}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/panoramic_mandible_results_v2.pdf}
    \caption{Jaccard Score of experiments with Panoramic Mandible Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:panoramic_mandible_results}
\end{figure*}
% Results Panoramic Mandible.

% \subsubsection{UFBA-UESC: Teeth}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/ufba_teeth_results_v2.pdf}
    \caption{Jaccard Score of experiments with UFBA-UESC Teeth Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:ufba_teeth_results}
\end{figure*}
% Results UFBA-UESC Teeth.

Excluding the target class, only 1 out of 12 tasks is from a DRX dataset. Being the most uncommon type of dataset in our experiments, they have less presence in the meta-training process. This corroborate with our hypotheses that the \protomethod method benefits from similar tasks in training, which explain the relative poor performance of this method in these type of tasks. 
One can notice a special poor performance for the Regions Type annotation for the \textit{UFBA-UESC Teeth} task (Figure~\ref{fig:ufba_teeth_results}). Our approach to generate these types of annotation appears too strict by only considering \textit{pure regions} (regions within a single class). The resulted superpixels from the SLIC algorithm, most likely included pixels from both classes given characteristics of the target class. Consequently no \textit{pure regions} for the \textit{Teeth} class are generated and selected, which makes the creation of prototypes for this class impossible and explain the approximately zero score. 



\subsubsection{Agricultural Tasks}\label{sec:agriculture_results}
In general, all Remote Sensing experiments show to be much more difficult than the Medical cases. Overall, no method achieved a Jaccard score above $0.8$ in any of the evaluated tasks, not even using dense labels.

For the agricultural tasks, we observe that the \mamlmethod method consistently outperform the fine-tuning and from scratch baselines, specially in the configurations with the lower amount of data (1-shot tasks). Although being related tasks, the \textit{Coffee} tasks have an intrinsically domain-shit between the different counties in the dataset. The geography of the cities differ, and the methods of plantation can be different. This explain why fine-tuning is not always the best solution. In Figures~\ref{fig:mon_results} and~\ref{fig:arc_results} we see the results for the \textit{Montesanto} and \textit{Arceburgo Coffee} task, from the Brazilian Coffee Dataset, while in Figure~\ref{fig:lrj_results} we present the results for the \textit{Orange Orchard} task.

% \subsubsection{Brazilian Coffee: Montesanto}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/montesanto_results_v2.pdf}
    \caption{Jaccard Score of experiments with Montesanto Coffee Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:mon_results}
\end{figure*}

% Results montesanto.

% \subsubsection{Brazilian Coffee: Arceburgo}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/arceburgo_results_v2.pdf}
    \caption{Jaccard Score of experiments with Arceburgo Coffee Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:arc_results}
\end{figure*}

% Results arceburgo.

% \subsubsection{Orange Orchards}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\currprop]{results/figs/laranja_results_v2.pdf}
    \caption{Jaccard Score of experiments with Orange Orchard Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
    \label{fig:lrj_results}
\end{figure*}
% Results oranges.

The \protomethod method had consistent results in most tasks. For the \textit{Coffee} tasks, it generally obtained a Jaccard score around $0.6$. For the \textit{Orange} task, it revolved around $0.4$ Jaccard. In a tendency similar to the Medical experiments, the \protomethod method seems to benefit from related/similar tasks. The \textit{Orange} task was unique in this set of tasks. When choosing \textit{Orange Orchard} as the target task, only the \textit{Coffee} tasks were available to be used in training. The absence of similar tasks appears to affect the \protomethod method results.

% \subsubsection{INRIA Tasks}\label{sec:inria_results}

% The INRIA Tasks presents a challenge that although the target class is the same in all tasks, each city have unique characteristics that differentiate them from each other. Also, the intrinsically variability in the target class \textit{Building} increases the difficulty for these tasks.

% As before, the \protomethod method remained consistent across different tasks and settings. Given the domain-shifts between tasks, surprisingly, it was the best method in practically all tasks, sometimes with large difference to the second-best method. In Figures~\ref{fig:austin_results}, \ref{fig:kitsap_results}, and \ref{fig:vienna_results}, we see the results for the \textit{Austin, Kitsap County}, and \textit{Vienna Building} tasks, respectively.

% % \subsubsection{Austin}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/austin_results.pdf}
%     \caption{Jaccard Score of experiments with Austin Building Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:austin_results}
% \end{figure*}
% % Results austin.

% % \subsubsection{Kitsap}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/kitsap_results.pdf}
%     \caption{Jaccard Score of experiments with Kitsap County Building Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:kitsap_results}
% \end{figure*}
% % Results kitsap.

% % \subsubsection{Vienna}
% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/vienna_results.pdf}
%     \caption{Jaccard Score of experiments with Vienna Building Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:vienna_results}
% \end{figure*}
% % Results kitsap.

% In most cases being the second-best, the \mamlmethod method outperform the \textit{From Scratch} baseline, and at least one of the fine-tuning baselines in most tasks. Again, with the difference within cities, the \mamlmethod method showed to be better as a starting point to fine-tune for a few-shot task than pre-training the model in a highly different dataset.

% Different from the Medical Experiments, as mentioned in the section~\ref{sec:ev_protocol}, we used $200$ epoch for the meta-training of the \mamlmethod and \protomethod methods. We argue that these methods did not fully converge with this number of training epochs, but we choose this number of epochs in order to evaluate a large number of tasks in a limited time. Moreover, there was no hyperparameter optimization. We tested the a configuration of hyperparameters (mentioned in Section~\ref{sec:ev_protocol}) with a single medical experiment, which seemed to converge, and used these same hyperparameters for all tasks. That said, as seen in the Medical Experiments (section~\ref{sec:med_results}), we expect that with proper hyperparameters and number of epochs, our methods achieve better results than currently have shown, specially for the ISPRS tasks (Section~\ref{sec:isprs_results}) that will be show next.

% \subsubsection{ISPRS Tasks}\label{sec:isprs_results}

% The ISPRS tasks have their own challenges and had the most surprising results. First, the two cities, Potsdam and Vaihingen, used different spectral bands. For Potsdam we used RGB images, and for Vaihingen we used NIRG images. This difference increases the natural domain-shift between different locations. Besides that, the tasks only have one other task with the same target class, which is in a different city. This shift implies that a same class will have different features in each of the cities. 

% In Figure~\ref{fig:vaihingen_road_results} we show the results for the \textit{Vaihingen Road} task, while in Figure~\ref{fig:vaihingen_tree_results} we present the results for the \textit{Vaihingen Tree} task. Meanwhile, in Figures~\ref{fig:postdam_road_results} and \ref{fig:postdam_building_results} we show the results for the \textit{Potsdam Road} task and \textit{Potsdam Building} task, respectively. Note that for the tasks \textit{Vaihingen Tree} and \textit{Potsdam Building}, only the \textit{From Scratch} baseline are presented.

% Given the difference between tasks, we expected that \mamlmethod~would be the best approach for the tasks. However, this was not the case for most of the tasks tested. Unexpectedly, the \textit{From Scratch} baseline, specially with dense annotations, obtained higher Jaccard scores than the other methods, with a few exceptions were it performs worse than or equivalent to the \mamlmethod. This is most noticeable for the tasks \textit{Vaihingen Tree} (Figure~\ref{fig:vaihingen_tree_results}) and \textit{Potsdam Building} (Figure~\ref{fig:postdam_building_results}). For the two tasks with Fine-tuning baselines, these baselines were in most cases the best performing, even when the source task was from the other city. Interestingly, for the \textit{Potsdam Roads} task (Figure~\ref{fig:postdam_road_results}), all methods had similar results around the $0.4$ Jaccard score independent of sparsity of shot number, with some clear exceptions. 

% Again, the \protomethod~ remained consistent for different tasks configurations. The Jaccard score achieved in the tasks were around $0.4$ in most of them. Once more, the absence of similar tasks, and the intravariability of some of the classes in the experiments, probably affected the results of the method.

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/vaihingen_road_results.pdf}
%     \caption{Jaccard Score of experiments with Vaihingen Roads Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:vaihingen_road_results}
% \end{figure*}
% % Results Vaihingen road.

% % \subsubsection{Vaihingen: Trees}
% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/vaihingen_tree_results.pdf}
%     \caption{Jaccard Score of experiments with Vaihingen Tree Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:vaihingen_tree_results}
% \end{figure*}
% % Results Vaihingen tree.

% % \subsubsection{Potsdam: Buildings}
% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/postdam_building_results.pdf}
%     \caption{Jaccard Score of experiments with Potsdam Buildings Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:postdam_building_results}
% \end{figure*}
% % Results Potsdam building.

% % \subsubsection{Potsdam: Roads}
% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/postdam_road_results.pdf}
%     \caption{Jaccard Score of experiments with Potsdam Roads Task.}% Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
%     \label{fig:postdam_road_results}
% \end{figure*}

% % \subsubsection{Vaihingen: Roads}

% % Results Potsdam road.

% % \subsubsection{Brazilian Coffee: Guaxupé}
% % \begin{figure*}[h]
% %     \centering
% %     \includegraphics[width=\columnwidth]{results/figs/guaxupe_results.pdf}
% %     \caption{Jaccard Score of experiments with Guaxupé Coffee Task. Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
% %     \label{fig:gux_results}
% % \end{figure*}

% % Results guaxupe.

% % \subsubsection{Brazilian Coffee: Guaranésia}
% % \begin{figure*}[h]
% %     \centering
% %     \includegraphics[width=\columnwidth]{results/figs/guaranesia_results.pdf}
% %     \caption{Jaccard Score of experiments with Guaranésia Coffee Task. Results are grouped by sparse annotation type and number of shots. Dashed lines are the scores of the methods trained with dense annotations.}
% %     \label{fig:gua_results}
% % \end{figure*}

% % Results guaranesia.

\subsection{Sparse Label Comparison}\label{sec:sparse_comparison}

In this section we show the results for our sparse annotations types comparisons. We choose some tasks, with multiple configurations, to compare the number of user inputs and the scores of our approaches. 
With these experiments we want to answer the second research question, for at least some of the sparse annotations evaluated in this work. 

In this section we only compared three types of sparse annotations: Points, Grid, and Regions. 
We defined the number of user inputs for a type of annotation as, the number of interactions an annotator would have to perform in order to sparsely annotate the image using said type. For a single image we defined the number of inputs for a n-point Points annotation simply as $2n$, since the user will select $n$ positive and $n$ negative pixels. For the Grid annotation, we define the number of inputs as the total positive labeled pixels in the grid, since all the pixels are assumed to be negative and the user pick the positive ones. And for the Regions annotation, the number of inputs is defined as the total regions selected, independent of being positive or negative. Once computed the number of inputs for a single image, we sum the values for all images in the support set of the $k$-shot task. Finally, we average the number of inputs of the $k$-shot across the five folds.

Figures~\ref{fig:inp_jsrt_results}, \ref{fig:inp_montesanto_results} present results label efficiency plots for \textit{JSRT Lungs} and \textit{Montesanto Coffee}, respectively. 
% In Figures~\ref{fig:inp_jsrt_results}, \ref{fig:inp_montesanto_results}, \ref{fig:inp_austin_results}, and \ref{fig:inp_vaihingen_results}, we present the results for the \textit{JSRT Lungs}, \textit{Montesanto Coffee}, \textit{Austin Buildings}, and \textit{Vaihingen Buildings}, respectively. 

\renewcommand{\currprop}{0.95\columnwidth}

% \subsection{JSRT: Lungs}
\begin{figure}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/inputs_jsrt_lungs.pdf}
    \caption{Number of user Inputs versus Jaccard Score in the JSRT Lungs Task.}
    \label{fig:inp_jsrt_results}
\end{figure}
% Results input JSRT.

% \subsection{Brazilian Coffee: Montesanto}
\begin{figure}[h]
    \centering
    \includegraphics[width=\currprop]{results/figs/inputs_mon_coffee.pdf}
    \caption{Number of user Inputs versus Jaccard Score in the Montesanto Coffee Task.}
    \label{fig:inp_montesanto_results}
\end{figure}
% Results input Montesanto.

% \subsection{Austin: Buildings}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/inputs_austin_building.pdf}
%     \caption{Number of user Inputs versus Jaccard Score in the Austin Buildings Task.}
%     \label{fig:inp_austin_results}
% \end{figure}
% % Results input Austin.

% % \subsection{Vaihingen: Buildings}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\currprop]{results/figs/inputs_vaihingen_building.pdf}
%     \caption{Number of user Inputs versus Jaccard Score in the Vaihingen Buildings Task.}
%     \label{fig:inp_vaihingen_results}
% \end{figure}
% Results input Vaihingen.

We observe that, as seen in the Section~\ref{sec:sparse_v_dense}, the \mamlmethod method overall performs better with more data information, that increases with the number of user inputs. We also, clearly see how the \protomethod method is almost indifferent to the sparsity and quantity of annotations by having a low deviation score in the presented tasks. 

For the \textit{JSRT Lungs} task (Figure~\ref{fig:inp_jsrt_results}), and Medical tasks, in general, we see that the Grid annotation usually achieve the higher score for the same number of user inputs as the other types of annotation. On the other hand, the Region annotation is commonly the best type of annotation for the Remote Sensing tasks, having higher scores with the same number of inputs. The Points annotation is, at most times, the worse performer. This was expected, since that with the same number of inputs this type of annotation will have less labeled pixels in total than the other types.

By comparing these results and the ones of the previous section (Section~\ref{sec:sparse_v_dense}) we can draw some conclusions. The Grid annotation is a solid annotation type that can lead to good results, and usually is one of the best types for the Medical cases. However, this is the most user consuming type, requiring the larger number of user inputs. The Regions annotation is also a solid option for annotation. When the superpixel segmentation produce clean regions easier to be labeled, this type can make the process of annotation simpler and quicker and produce precise models, specially for Remote Sensing tasks. The Points annotation is the easier to implement and require less from the user. Is does not produce the most optimal models, but can lead to comparable results requiring far less inputs. Also this annotation, guarantee a balanced number of pixels samples for each class in training, which can make optimization of the models easier. The other two types of annotations, Contours and Skeletons, appears as valid options as well. The way we designed the process of generating this annotations made it difficult to translate to a countable user input, which is the motive this types are not compared in this section. However, the results presented in Section~\ref{sec:sparse_v_dense}, show that both, Contours and Skeletons annotations, are suitable styles, specially Contours in the Medical tasks and Skeletons in Remote Sensing tasks.



% \subsection{WeaSeL Fast Adaptation}\label{sec:adapt_time}
% In this section we present the results for the adaptation time required by the \mamlmethod and a Fine-tuning baseline in some selected tasks.

% For this experiments we want to evaluate the number of epochs that the models required to converge in the few-shot task tuning phase. For this we executed a small experiment. We trained the models using the \mamlmethod method and using a source dataset. The models were trained for $200$ epochs and at epoch $100$ and $200$ we used the trained weights, at that epoch, as starting points to fine-tune to a few-shot task. Them we observe the Jaccard score for each fine-tune epoch until the epoch $50$, where we stopped tuning. 

% In Figures~\ref{fig:epoch_score_openist_lungs} and \ref{fig:epoch_score_inbreast_breast} we present the results of the \textit{OpenIST Lungs} and \textit{INbreast Breast} tasks, respectively. Figures~\ref{fig:epoch_score_mon_coffee}, \ref{fig:epoch_score_arc_coffee} and \ref{fig:epoch_score_lrj_laranja} contains the results of \textit{Montesanto Coffee}, \textit{Arceburgo Coffee}, and \textit{Orange Orchard} tasks, in that order. In the graphs we marked with a vertical line the epoch $40$. This epoch is were the few-shot tuning of the Remote Sensing tasks was stopped and is half the number of epochs used for the few-shot tuning in the Medical tasks. Also, the numbers over the small graphs represent the number of shots and sparse parameter of the annotation type used, for example, in the top-right graph in Figure~\ref{fig:epoch_score_inbreast_breast} is the $1$-shot \textit{INbreast Breast} task with $20$-point annotation. 

% As already discussed in Section~\ref{sec:sparse_v_dense}, the number of epochs of pre-training is not sufficient to converge with the \mamlmethod approach. This condition can makes our analyzes of these results less conclusive. Regardless, is clear observing the graphs, the instability of the scores in most cases. This indicate that the models did not fully converge to the few-shot task in the epoch span chosen. Also, we observe that the curves of the \mamlmethod method and the Fine-tuning baselines have a similar behavior in most cases. These two observations lead us to believe that the \textit{fast adaptation} of the MAML method did not occur in our experiments. This result can be from the lack of convergence in pre-training due to small number of epochs, or this expected feature of the method simply is not possible with our tested cases. 

% % \subsection{OpenIST: Lungs}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_openist_lungs_contours.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the OpenIST Lungs task using Contours annotation.}
%     \label{fig:epoch_score_openist_lungs}
% \end{figure}
% % \subsection{Inbreast: Breast}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_inbreast_breast_points.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the INbreast Breast task using Points annotation.}
%     \label{fig:epoch_score_inbreast_breast}
% \end{figure}
% % \subsection{Brazilian Coffee: Montesanto}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_mon_coffee_skels.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the Montesanto Coffee task using Skeletons annotation.}
%     \label{fig:epoch_score_mon_coffee}
% \end{figure}
% % \subsection{Brazilian Coffee: Arceburgo}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_arc_coffee_regions.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the Arceburgo Coffee task using Regions annotation.}
%     \label{fig:epoch_score_arc_coffee}
% \end{figure}
% % \subsection{Orange Orchard}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_lrj_laranja_points.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the Orange Orchard task using Points annotation.}
%     \label{fig:epoch_score_lrj_laranja}
% \end{figure}
% \subsection{Chicago: Buildings}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_openist_lungs_contours.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the OpenIST Lungs task using Contours annotation.}
%     \label{fig:epoch_score_openist_lungs}
% \end{figure}
% \subsection{Vaihingen: Roads}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{results/figs/epoch_score_openist_lungs_contours.pdf}
%     \caption{Jaccard Score by few-shot fine-tuning Epoch in the OpenIST Lungs task using Contours annotation.}
%     \label{fig:epoch_score_openist_lungs}
% \end{figure}
